Mixing and sharpening at the interface of a two-layer fluid forced by random jets

Understanding mixing at density interfaces is essential for predicting transport in stratified environmental flows. Laboratory studies have mostly relied on steady, spatially uniform forcing, whereas turbulence in nature is intermittent and heterogeneous. Here, we present experiments on a two-layer salt-stratified fluid forced by random turbulent bursts generated with a randomly actuated synthetic jet array (RASJA). Density fields are recorded with the light attenuation technique, allowing us to resolve the interface evolution. We measure that the upward velocity of the interface decreases with the density jump, in agreement with the power-law found in previous oscillating-grid studies. At large density differences, the interface sharpens during mixing, contrary to the smaller density jump case. Background potential energy analysis demonstrates irreversible mixing in both cases, with comparable energy changes. These results extend classical laboratory observations to a more isotropic forcing, offering new insights into the dynamics of mixing in geophysical settings.

==> thebibliography <==
\begin{thebibliography}{99}

\bibitem{ponder_sedimentation_1925}
E.~Ponder,
\newblock ``On sedimentation and rouleaux formation,''
\newblock \emph{Quarterly Journal of Experimental Physiology},
\newblock 1925.

\bibitem{batchelor_sedimentation_1972}
G.~K. Batchelor,
\newblock ``Sedimentation in a dilute dispersion of spheres,''
\newblock \emph{Journal of Fluid Mechanics},
\newblock vol.~52,
\newblock no.~2,
\newblock pp.~245--268,
\newblock 1972.

\bibitem{senis_settling_2001}
D.~Senis, L.~Talini, and C.~Allain,
\newblock ``Settling in aggregating colloidal suspensions,''
\newblock \emph{Oil \& Gas Science and Technology Rev IFP},
\newblock vol.~56,
\newblock no.~2,
\newblock pp.~153--159,
\newblock 2001.

\bibitem{ruffenach_diffusion_nodate}
W.~Ruffenach and R.~Volk,
\newblock ``Diffusion turbulente à travers une interface de densité (Turbulent diffusion through a density interface),''
\newblock Poster,
\newblock 2023.

\bibitem{gostiaux_diffusion_2013}
L.~Gostiaux, A.~Venaille, and J.~Sommeria,
\newblock ``Diffusion turbulente à travers une interface de densité : observations expérimentales et approche statistique,''
\newblock In \emph{Bordeaux, France},
\newblock 2013.
\newblock \url{https://hal.archives-ouvertes.fr/hal-03439784}.

\bibitem{laplace_etude_2022}
B.~Laplace,
\newblock ``Etude expérimentale de la sédimentation de particules intertielles en turbulence,''
\newblock PhD thesis,
\newblock Ecole Normale Supérieure de Lyon,
\newblock Université de Lyon,
\newblock 2022.

\bibitem{machicoane_particules_2014}
N.~Machicoane,
\newblock ``Particules matérielles en écoulement turbulent. Transport, dynamique aux temps longs et transfert thermique,''
\newblock PhD thesis,
\newblock Ecole Normale Supérieure de Lyon,
\newblock Université de Lyon,
\newblock 2014.

\bibitem{basset_lagrangian_2023}
T.~Basset,
\newblock ``Lagrangian investigation of particle dispersion in turbulence,''
\newblock PhD thesis,
\newblock Ecole Normale Supérieure de Lyon,
\newblock Université de Lyon,
\newblock 2023.

\bibitem{guazzelli_fluctuations_2011}
É.~Guazzelli and J.~Hinch,
\newblock ``Fluctuations and instability in sedimentation,''
\newblock \emph{Annual Review of Fluid Mechanics},
\newblock vol.~43,
\newblock no.~1,
\newblock pp.~97--116,
\newblock 2011.
\newblock \url{https://www.annualreviews.org/doi/10.1146/annurev-fluid-122109-160736}.

\bibitem{firouzi_quantitative_2015}
Mahshid Firouzi, Tony Howes, and Anh~V. Nguyen,
\newblock ``A quantitative review of the transition salt concentration for inhibiting bubble coalescence,''
\newblock \emph{Advances in Colloid and Interface Science},
\newblock vol.~222,
\newblock pp.~305--318,
\newblock 2015.
\newblock \url{https://linkinghub.elsevier.com/retrieve/pii/S0001868614002292}.

\bibitem{fernando_note_1993}
H.~J.~S. Fernando and I.~P.~D. De Silva,
\newblock ``Note on secondary flows in oscillating-grid, mixing-box experiments,''
\newblock \emph{Physics of Fluids A: Fluid Dynamics},
\newblock vol.~5,
\newblock no.~7,
\newblock pp.~1849--1851,
\newblock 1993.
\newblock \url{https://pubs.aip.org/pof/article/5/7/1849/441585/Note-on-secondary-flows-in-oscillating-grid-mixing}.

\bibitem{kraichnan_relation_1964}
R.~H. Kraichnan,
\newblock ``Relation between lagrangian and eulerian correlation times of a turbulent velocity field,''
\newblock \emph{The Physics of Fluids},
\newblock vol.~7,
\newblock no.~1,
\newblock pp.~142--143,
\newblock 1964.
\newblock \url{https://pubs.aip.org/pfl/article/7/1/142/832564/Relation-between-Lagrangian-and-Eulerian}.

\bibitem{laplace_suspension_2023}
B.~Laplace, J.~Vessaire, O.~Tolfts, M.~Bourgoin, and R.~Volk,
\newblock ``Suspension of large inertial particles in a turbulent swirling flow,''
\newblock \emph{Physical Review Fluids},
\newblock vol.~8,
\newblock no.~6,
\newblock p.~064301,
\newblock 2023.
\newblock \url{https://link.aps.org/doi/10.1103/PhysRevFluids.8.064301}.

\bibitem{machicoane_simplified_2019}
N.~Machicoane, A.~Aliseda, R.~Volk, and M.~Bourgoin,
\newblock ``A simplified and versatile calibration method for multi-camera optical systems in 3d particle imaging,''
\newblock \emph{Review of Scientific Instruments},
\newblock vol.~90,
\newblock no.~3,
\newblock p.~035112,
\newblock 2019.
\newblock \url{https://pubs.aip.org/rsi/article/90/3/035112/359348/A-simplified-and-versatile-calibration-method-for}.

\bibitem{machicoane_large_2014}
N.~Machicoane, R.~Zimmermann, L.~Fiabane, M.~Bourgoin, J.-F. Pinton, and R.~Volk,
\newblock ``Large sphere motion in a nonhomogeneous turbulent flow,''
\newblock \emph{New Journal of Physics},
\newblock vol.~16,
\newblock no.~1,
\newblock p.~013053,
\newblock 2014.
\newblock \url{https://iopscience.iop.org/article/10.1088/1367-2630/16/1/013053}.

\bibitem{maxey_velocity_1987}
M.~R. Maxey,
\newblock ``The velocity skewness measured in grid turbulence,''
\newblock \emph{The Physics of Fluids},
\newblock vol.~30,
\newblock no.~4,
\newblock pp.~935--938,
\newblock 1987.
\newblock \url{https://pubs.aip.org/pfl/article/30/4/935/846565/The-velocity-skewness-measured-in-grid}.

\bibitem{schanz_shake--box_2016}
D.~Schanz, S.~Gesemann, and A.~Schröder,
\newblock ``Shake-the-box: lagrangian particle tracking at high particle image densities,''
\newblock \emph{Experiments in Fluids},
\newblock vol.~57,
\newblock no.~5,
\newblock p.~70,
\newblock 2016.
\newblock \url{http://link.springer.com/10.1007/s00348-016-2157-1}.

\bibitem{seyed-ahmadi_sedimentation_2021}
A.~Seyed-Ahmadi and A.~Wachs,
\newblock ``Sedimentation of inertial monodisperse suspensions of cubes and spheres,''
\newblock \emph{Physical Review Fluids},
\newblock vol.~6,
\newblock no.~4,
\newblock p.~044306,
\newblock 2021.
\newblock \url{https://link.aps.org/doi/10.1103/PhysRevFluids.6.044306}.

\bibitem{variano_random-jet-stirred_2008}
E.~A. Variano and E.~A. Cowen,
\newblock ``A random-jet-stirred turbulence tank,''
\newblock \emph{Journal of Fluid Mechanics},
\newblock vol.~604,
\newblock pp.~1--32,
\newblock 2008.
\newblock \url{https://www.cambridge.org/core/product/identifier/S0022112008000645/type/journal_article}.

\bibitem{fernando_turbulent_1991}
H.~J.~S. Fernando,
\newblock ``Turbulent mixing in stratified fluids,''
\newblock \emph{Annual Review of Fluid Mechanics},
\newblock vol.~23,
\newblock no.~1,
\newblock pp.~455--493,
\newblock 1991.
\newblock \url{https://www.annualreviews.org/doi/10.1146/annurev.fl.23.010191.002323}.

\bibitem{venaille_dynamical_2007}
A.~Venaille and J.~Sommeria,
\newblock ``A dynamical equation for the distribution of a scalar advected by turbulence,''
\newblock \emph{Physics of Fluids},
\newblock vol.~19,
\newblock no.~2,
\newblock p.~028101,
\newblock 2007.
\newblock \url{https://pubs.aip.org/pof/article/19/2/028101/255560/A-dynamical-equation-for-the-distribution-of-a}.

\bibitem{venaille_statistical_2017}
A.~Venaille, L.~Gostiaux, and J.~Sommeria,
\newblock ``A statistical mechanics approach to mixing in stratified fluids,''
\newblock \emph{Journal of Fluid Mechanics},
\newblock vol.~810,
\newblock pp.~554--583,
\newblock 2017.
\newblock \url{https://www.cambridge.org/core/product/identifier/S0022112016007217/type/journal_article}.

\bibitem{rouse_diffusion_1955}
H.~Rouse and J.~Dodu,
\newblock ``Diffusion turbulente à travers une discontinuité de densité,''
\newblock \emph{La Houille Blanche},
\newblock vol.~41,
\newblock no.~4,
\newblock pp.~522--532,
\newblock 1955.
\newblock \url{https://www.tandfonline.com/doi/full/10.1051/lhb/1955050}.

\bibitem{caulfield_layering_2021}
C.~P. Caulfield,
\newblock ``Layering, instabilities, and mixing in turbulent stratified flows,''
\newblock \emph{Annual Review of Fluid Mechanics},
\newblock vol.~53,
\newblock no.~1,
\newblock pp.~113--145,
\newblock 2021.
\newblock \url{https://www.annualreviews.org/doi/10.1146/annurev-fluid-042320-100458}.

\bibitem{allgayer_application_2012}
D.~M. Allgayer and G.~R. Hunt,
\newblock ``On the application of the light-attenuation technique as a tool for non-intrusive buoyancy measurements,''
\newblock \emph{Experimental Thermal and Fluid Science},
\newblock vol.~38,
\newblock pp.~257--261,
\newblock 2012.
\newblock \url{https://linkinghub.elsevier.com/retrieve/pii/S0894177711002287}.

\bibitem{petropoulos_settling_2023}
N.~Petropoulos, C.~P. Caulfield, P.~Meunier, and E.~Villermaux,
\newblock ``Settling versus mixing in stratified shear flows,''
\newblock \emph{Journal of Fluid Mechanics},
\newblock vol.~974,
\newblock p.~R1,
\newblock 2023.
\newblock \url{https://www.cambridge.org/core/product/identifier/S0022112023008042/type/journal_article}.

\bibitem{davies_wykes_meaning_2015}
M.~S. Davies Wykes, G.~O. Hughes, and S.~B. Dalziel,
\newblock ``On the meaning of mixing efficiency for buoyancy-driven mixing in stratified turbulent flows,''
\newblock \emph{Journal of Fluid Mechanics},
\newblock vol.~781,
\newblock pp.~261--275,
\newblock 2015.
\newblock \url{https://www.cambridge.org/core/product/identifier/S0022112015004620/type/journal_article}.

\bibitem{bartello_sensitivity_2013}
P.~Bartello and S.~M. Tobias,
\newblock ``Sensitivity of stratified turbulence to the buoyancy reynolds number,''
\newblock \emph{Journal of Fluid Mechanics},
\newblock vol.~725,
\newblock pp.~1--22,
\newblock 2013.
\newblock \url{https://www.cambridge.org/core/product/identifier/S0022112013001705/type/journal_article}.

\bibitem{holford_measurements_1996}
J.~M. Holford and S.~B. Dalziel,
\newblock ``Measurements of layer depth during baroclinic instability in a two-layer flow,''
\newblock \emph{Applied Scientific Research},
\newblock vol.~56,
\newblock no.~2,
\newblock pp.~191--207,
\newblock 1996.
\newblock \url{https://doi.org/10.1007/BF02249381}.

\bibitem{park_turbulent_1994}
Y.-G. Park, J.~A. Whitehead, and A.~Gnanadeskian,
\newblock ``Turbulent mixing in stratified fluids: layer formation and energetics,''
\newblock \emph{Journal of Fluid Mechanics},
\newblock vol.~279,
\newblock pp.~279--311,
\newblock 1994.
\newblock \url{https://www.cambridge.org/core/product/identifier/S0022112094003915/type/journal_article}.

\bibitem{dossmann_mixing_2017}
Y.~Dossmann, F.~Pollet, P.~Odier, and T.~Dauxois,
\newblock ``Mixing and formation of layers by internal wave forcing,''
\newblock \emph{Journal of Geophysical Research: Oceans},
\newblock vol.~122,
\newblock no.~12,
\newblock pp.~9906--9917,
\newblock 2017.
\newblock \url{https://onlinelibrary.wiley.com/doi/abs/10.1002/2017JC013309}.

\bibitem{howland_mixing_2020}
C.~J. Howland, J.~R. Taylor, and C.~P. Caulfield,
\newblock ``Mixing in forced stratified turbulence and its dependence on large-scale forcing,''
\newblock \emph{Journal of Fluid Mechanics},
\newblock vol.~898,
\newblock p.~A7,
\newblock 2020.
\newblock \url{https://www.cambridge.org/core/journals/journal-of-fluid-mechanics/article/mixing-in-forced-stratified-turbulence-and-its-dependence-on-largescale-forcing/8E92567661BD476111D7E19C6D1B1CF3#}.

\bibitem{cenedese_concentration_1998}
C.~Cenedese and S.~Dalziel,
\newblock ``Concentration and depth field determined by the light transmitted through a dyed solution,''
\newblock In \emph{Proceedings},
\newblock 1998.
\newblock \url{https://www.semanticscholar.org/paper/CONCENTRATION-AND-DEPTH-FIELD-DETERMINED-BY-THE-A-Cenedese-Dalziel/95e9a949d3ec30ce3592d317614dac5fd2382d31}.

\bibitem{scotti_diagnosing_2014}
A.~Scotti and B.~White,
\newblock ``Diagnosing mixing in stratified turbulent flows with a locally defined available potential energy,''
\newblock \emph{Journal of Fluid Mechanics},
\newblock vol.~740,
\newblock pp.~114--135,
\newblock 2014.
\newblock \url{https://www.cambridge.org/core/product/identifier/S0022112013006435/type/journal_article}.

\bibitem{mercier_plastic_2023}
M.~J. Mercier, M.~Poulain-Zarcos, Y.~Ourmiéres, J.~F. Ghiglione, and A.~Ter Halle,
\newblock ``Plastic litter in the oceans. Most of it has gone missing, but it might just be transformed… or transported,''
\newblock \emph{Europhysics News},
\newblock vol.~54,
\newblock no.~3,
\newblock pp.~24--27,
\newblock 2023.
\newblock \url{https://www.europhysicsnews.org/10.1051/epn/2023303}.

\bibitem{poulain-zarcos_global_2022}
M.~Poulain-Zarcos, M.~J. Mercier, and A.~Ter Halle,
\newblock ``Global characterization of oscillating grid turbulence in homogeneous and two-layer fluids, and its implication for mixing at high peclet number,''
\newblock \emph{Physical Review Fluids},
\newblock vol.~7,
\newblock no.~5,
\newblock p.~054606,
\newblock 2022.
\newblock \url{https://link.aps.org/doi/10.1103/PhysRevFluids.7.054606}.

\bibitem{poulain_distribution_2019}
M.~Poulain, A.~ter Halle, and M.~Mercier,
\newblock ``Distribution de particules en turbulence de surface : application à la pollution plastique océanique,''
\newblock In \emph{24e Congrès Français de Mécanique},
\newblock 2019.
\newblock \url{https://hal.science/hal-02406337}.

\bibitem{ourmieres_inferring_2023}
Y.~Ourmieres, M.~Arnaud, P.~Deixonne, J.-F. Ghiglione, M.~Albignac, M.~Poulain-Zarcos, M.~Mercier, and A.~Ter Halle,
\newblock ``Inferring microplastics origins in the mediterranean sea by coupling modelling and in-situ measurements,''
\newblock \emph{Marine Pollution Bulletin},
\newblock vol.~195,
\newblock p.~115333,
\newblock 2023.
\newblock \url{https://linkinghub.elsevier.com/retrieve/pii/S0025326X23007671}.

\bibitem{poulain_etude_2020}
M.~Poulain,
\newblock ``Etude de la distribution verticale de particules plastiques dans l'océan : caractérisation, modélisation et comparaison avec des observations,''
\newblock PhD thesis,
\newblock Institut National Polytechnique de Toulouse - INPT,
\newblock 2020.
\newblock \url{https://theses.hal.science/tel-04427024}.

\bibitem{bourget_ondes_2014}
B.~Bourget,
\newblock ``Ondes internes, de l'instabilité au mélange. Approche expérimentale,''
\newblock PhD thesis,
\newblock Ecole normale supérieure de lyon - ENS LYON,
\newblock 2014.
\newblock \url{https://theses.hal.science/tel-01073663}.

\bibitem{fondation_tara_ocean_livre_2020}
Fondation Tara Océan,
\newblock \emph{Le livre bleu de tara: aux sources de la pollution plastique.},
\newblock 2020.
\newblock \url{https://oceans.taraexpeditions.org/wp-content/uploads/2020/03/LivreBleu_Tara_Microplastiques2019.pdf}.

\bibitem{pohl_transport_2020}
F.~Pohl, J.~T. Eggenhuisen, I.~A. Kane, M.~A. Clare, and R.~Wogelius,
\newblock ``Transport and burial of microplastics in deep-marine sediments by turbidity currents,''
\newblock \emph{Environmental Science \& Technology},
\newblock vol.~54,
\newblock no.~7,
\newblock pp.~4180--4189,
\newblock 2020.
\newblock \url{https://pubs.acs.org/doi/10.1021/acs.est.9b07527}.

\bibitem{zinke_moving_2020}
L.~Zinke,
\newblock ``Moving marine microplastics,''
\newblock \emph{Nature Reviews Earth \& Environment},
\newblock vol.~1,
\newblock no.~4,
\newblock p.~186,
\newblock 2020.
\newblock \url{https://www.nature.com/articles/s43017-020-0047-9}.

\bibitem{kane_seafloor_2020}
I.~A. Kane, M.~A. Clare, E.~Miramontes, M.~A. Wogelius, J.~J. Rothwell, P.~Garreau, and F.~Pohl,
\newblock ``Seafloor microplastic hotspots controlled by deep-sea circulation,''
\newblock \emph{Science},
\newblock vol.~368,
\newblock no.~6495,
\newblock pp.~1140--1145,
\newblock 2020.
\newblock \url{https://www.science.org/doi/10.1126/science.aba5899}.

\bibitem{kane_dispersion_2019}
I.~A. Kane and M.~A. Clare,
\newblock ``Dispersion, accumulation, and the ultimate fate of microplastics in deep-marine environments: a review and future directions,''
\newblock \emph{Frontiers in Earth Science},
\newblock vol.~7,
\newblock p.~80,
\newblock 2019.
\newblock \url{https://www.frontiersin.org/article/10.3389/feart.2019.00080/full}.

\bibitem{park_exploring_2023}
S.~Park, I.~Kim, W.-H. Jeon, and H.~S. Moon,
\newblock ``Exploring the vertical transport of microplastics in subsurface environments: lab-scale experiments and field evidence,''
\newblock \emph{Journal of Contaminant Hydrology},
\newblock vol.~257,
\newblock p.~104215,
\newblock 2023.
\newblock \url{https://linkinghub.elsevier.com/retrieve/pii/S0169772223000852}.

\bibitem{brach_anticyclonic_2018}
Laurent Brach, Patrick Deixonne, Marie-France Bernard, Edmée Durand, Marie-Christine Desjean, Emile Perez, Erik Van Sebille, and Alexandra Ter Halle,
\newblock ``Anticyclonic eddies increase accumulation of microplastic in the north atlantic subtropical gyre,''
\newblock \emph{Marine Pollution Bulletin},
\newblock vol.~126,
\newblock pp.~191--196,
\newblock 2018.
\newblock \url{https://linkinghub.elsevier.com/retrieve/pii/S0025326X17309232}.

\bibitem{phillips_turbulence_1972}
O.~M. Phillips,
\newblock ``Turbulence in a strongly stratified fluid—is it unstable?,''
\newblock \emph{Deep Sea Research and Oceanographic Abstracts},
\newblock vol.~19,
\newblock no.~1,
\newblock pp.~79--81,
\newblock 1972.
\newblock \url{https://linkinghub.elsevier.com/retrieve/pii/0011747172900745}.

\bibitem{posmentier_generation_1977}
Eric~S. Posmentier,
\newblock ``The generation of salinity finestructure by vertical diffusion,''
\newblock \emph{Journal of Physical Oceanography},
\newblock vol.~7,
\newblock no.~2,
\newblock pp.~298--300,
\newblock 1977.
\newblock \url{http://journals.ametsoc.org/doi/10.1175/1520-0485(1977)007<0298:TGOSFB>2.0.CO;2}.

\bibitem{venaille_role_2014}
A.~Venaille, L.~Gostiaux, and J.~Sommeria,
\newblock ``The role of fluctuations across a density interface,''
\newblock 2014.
\newblock \url{https://arxiv.org/abs/1409.6010}.

\end{thebibliography}

